A population analysis of pulse broadening in ASKAP Fast Radio Bursts

The pulse morphology of fast radio bursts (FRBs) provides key information in both understanding progenitor physics and the plasma medium through which the burst propagates. We present a study of the profiles of 33 bright FRBs detected by the Australian Square Kilometre Array Pathfinder. We identify seven FRBs with measureable intrinsic pulse widths, including two FRBs that have been seen to repeat. In our modest sample we see no evidence for bimodality in the pulse width distribution. We also identify five FRBs with evidence of millisecond timescale pulse broadening caused by scattering in inhomogeneous plasma. We find no evidence for a relationship between pulse broadening and extragalactic dispersion measure. The scattering could be either caused by extreme turbulence in the host galaxy or chance propagation through foreground galaxies. With future high time resolution observations and detailed study of host galaxy properties we may be able to probe line-of-sight turbulence on gigaparsec scales.

==> backupscatfit.tex <==
170107 & $608.40_{-0.87}^{+0.83}$ & $1.10_{-0.24}^{+0.25}$ & < 3.50&$-2.12\pm0.46$ \\
170416 & $523.70_{-0.49}^{+0.48}$ & $2.41_{-0.28}^{+0.32}$ & < 3.74&$-2.51\pm0.47$ \\
170428 & $992.48_{-0.75}^{+0.69}$ & $<1.16$ & < 3.58&$-2.66\pm0.46$ \\
170707 & $233.92_{-0.88}^{+0.81}$ & $2.00_{-0.31}^{+0.34}$ & < 6.53&$-1.96\pm0.45$ \\
170712 & $312.40_{-0.28}^{+0.31}$ & $0.82_{-0.15}^{+0.14}$ & < 2.25&$-2.86\pm0.46$ \\
170906 & $391.00_{-0.23}^{+0.23}$ & $1.08_{-0.13}^{+0.12}$ & < 1.40&$-3.37\pm0.47$ \\
171003 & $465.08_{-0.25}^{+0.24}$ & $0.94_{-0.14}^{+0.15}$ & < 1.87&$-2.73\pm0.46$ \\
171004 & $303.80_{-0.33}^{+0.34}$ & $1.00_{-0.21}^{+0.20}$ & < 3.31&$-2.88\pm0.45$ \\
171019 & $461.99_{-0.57}^{+0.58}$ & $2.88_{-0.14}^{+0.14}$ & < 3.52&$-1.00\pm0.50$ \\
171020 & $113.94_{-0.15}^{+0.13}$ & $0.82_{-0.15}^{+0.09}$ & < 1.21&$-3.05\pm0.47$ \\
171116 & $618.15_{-0.42}^{+0.43}$ & $1.47_{-0.26}^{+0.27}$ & < 4.70&$-2.24\pm0.45$ \\
171213 & $158.43_{-0.10}^{+0.08}$ & $0.70_{-0.20}^{+0.12}$ & < 1.45&$-3.51\pm0.47$ \\
171216 & $203.84_{-0.33}^{+0.32}$ & $1.16_{-0.20}^{+0.24}$ & < 1.94&$-3.37\pm0.46$ \\
180110 & $714.04_{-0.25}^{+0.26}$ & $0.61_{-0.30}^{+0.28}$ & $16.84_{-0.75}^{+0.76}$&$140.14\pm0.47$ \\
180119 & $401.43_{-0.23}^{+0.23}$ & $0.41_{-0.20}^{+0.23}$ & $5.43_{-0.82}^{+0.89}$&$15.21\pm0.46$ \\
180128.0 & $441.33_{-0.45}^{+0.45}$ & $1.35_{-0.22}^{+0.23}$ & < 4.98&$-0.58\pm0.45$ \\
180128.2 & $495.20_{-0.62}^{+0.50}$ & $0.57_{-0.30}^{+0.27}$ & $6.38_{-1.05}^{+1.18}$&$4.50\pm0.49$ \\
180130 & $343.24_{-0.72}^{+0.76}$ & $0.84_{-0.47}^{+0.48}$ & $15.74_{-3.15}^{+3.39}$&$10.99\pm0.45$ \\
180131 & $657.45_{-0.53}^{+0.53}$ & $2.31_{-0.29}^{+0.29}$ & < 6.77&$-0.81\pm0.45$ \\
180212 & $167.52_{-0.13}^{+0.12}$ & $0.73_{-0.16}^{+0.11}$ & < 0.97&$-4.06\pm0.47$ \\
180315 & $478.90_{-0.39}^{+0.36}$ & $0.67_{-0.34}^{+0.29}$ & < 1.52&$-2.96\pm0.46$ \\
180324 & $429.73_{-0.34}^{+0.34}$ & $0.79_{-0.35}^{+0.37}$ & $7.85_{-1.60}^{+1.67}$&$4.44\pm0.46$ \\
180417 & $474.65_{-0.15}^{+0.13}$ & $1.04_{-0.07}^{+0.07}$ & < 1.40&$-3.14\pm0.47$ \\
180430 & $264.10_{-0.03}^{+0.03}$ & $0.68_{-0.20}^{+0.12}$ & < 0.77&$-4.43\pm0.50$ \\
180515 & $354.86_{-0.21}^{+0.17}$ & $0.74_{-0.28}^{+0.24}$ & < 1.79&$-2.19\pm0.47$ \\
180525 & $387.57_{-0.15}^{+0.16}$ & $1.78_{-0.12}^{+0.13}$ & $3.75_{-0.58}^{+0.53}$&$5.22\pm0.48$ \\
180924 & $362.39_{-0.16}^{+0.16}$ & $0.75_{-0.10}^{+0.11}$ & < 2.28&$-1.61\pm0.47$ \\
181112 & $588.77_{-0.20}^{+0.19}$ & $0.57_{-0.14}^{+0.13}$ & < 1.71&$-4.36\pm0.47$ \\
190102 & $364.35_{-0.23}^{+0.21}$ & $0.45_{-0.20}^{+0.21}$ & < 1.69&$-2.44\pm0.46$ \\
190608 & $340.80_{-0.68}^{+0.64}$ & $2.30_{-0.59}^{+0.62}$ & $6.76_{-2.40}^{+2.07}$&$0.45\pm0.46$ \\
190611.2 & $321.29_{-0.89}^{+0.96}$ & $1.58_{-0.30}^{+0.30}$ & < 3.42&$-2.74\pm0.46$ \\
190711 & $590.46_{-0.73}^{+0.70}$ & $3.51_{-0.23}^{+0.24}$ & < 2.85&$-2.20\pm0.47$ \\
190714 & $503.86_{-0.31}^{+0.31}$ & $0.95_{-0.23}^{+0.19}$ & < 2.78&$-2.36\pm0.44$ \\

==> craft-scatter 200707/backupscatfit.tex <==
170107 & $608.40_{-0.87}^{+0.83}$ & $1.10_{-0.24}^{+0.25}$ & < 3.50&$-2.12\pm0.46$ \\
170416 & $523.70_{-0.49}^{+0.48}$ & $2.41_{-0.28}^{+0.32}$ & < 3.74&$-2.51\pm0.47$ \\
170428 & $992.48_{-0.75}^{+0.69}$ & $<1.16$ & < 3.58&$-2.66\pm0.46$ \\
170707 & $233.92_{-0.88}^{+0.81}$ & $2.00_{-0.31}^{+0.34}$ & < 6.53&$-1.96\pm0.45$ \\
170712 & $312.40_{-0.28}^{+0.31}$ & $0.82_{-0.15}^{+0.14}$ & < 2.25&$-2.86\pm0.46$ \\
170906 & $391.00_{-0.23}^{+0.23}$ & $1.08_{-0.13}^{+0.12}$ & < 1.40&$-3.37\pm0.47$ \\
171003 & $465.08_{-0.25}^{+0.24}$ & $0.94_{-0.14}^{+0.15}$ & < 1.87&$-2.73\pm0.46$ \\
171004 & $303.80_{-0.33}^{+0.34}$ & $1.00_{-0.21}^{+0.20}$ & < 3.31&$-2.88\pm0.45$ \\
171019 & $461.99_{-0.57}^{+0.58}$ & $2.88_{-0.14}^{+0.14}$ & < 3.52&$-1.00\pm0.50$ \\
171020 & $113.94_{-0.15}^{+0.13}$ & $0.82_{-0.15}^{+0.09}$ & < 1.21&$-3.05\pm0.47$ \\
171116 & $618.15_{-0.42}^{+0.43}$ & $1.47_{-0.26}^{+0.27}$ & < 4.70&$-2.24\pm0.45$ \\
171213 & $158.43_{-0.10}^{+0.08}$ & $0.70_{-0.20}^{+0.12}$ & < 1.45&$-3.51\pm0.47$ \\
171216 & $203.84_{-0.33}^{+0.32}$ & $1.16_{-0.20}^{+0.24}$ & < 1.94&$-3.37\pm0.46$ \\
180110 & $714.04_{-0.25}^{+0.26}$ & $0.61_{-0.30}^{+0.28}$ & $16.84_{-0.75}^{+0.76}$&$140.14\pm0.47$ \\
180119 & $401.43_{-0.23}^{+0.23}$ & $0.41_{-0.20}^{+0.23}$ & $5.43_{-0.82}^{+0.89}$&$15.21\pm0.46$ \\
180128.0 & $441.33_{-0.45}^{+0.45}$ & $1.35_{-0.22}^{+0.23}$ & < 4.98&$-0.58\pm0.45$ \\
180128.2 & $495.20_{-0.62}^{+0.50}$ & $0.57_{-0.30}^{+0.27}$ & $6.38_{-1.05}^{+1.18}$&$4.50\pm0.49$ \\
180130 & $343.24_{-0.72}^{+0.76}$ & $0.84_{-0.47}^{+0.48}$ & $15.74_{-3.15}^{+3.39}$&$10.99\pm0.45$ \\
180131 & $657.45_{-0.53}^{+0.53}$ & $2.31_{-0.29}^{+0.29}$ & < 6.77&$-0.81\pm0.45$ \\
180212 & $167.52_{-0.13}^{+0.12}$ & $0.73_{-0.16}^{+0.11}$ & < 0.97&$-4.06\pm0.47$ \\
180315 & $478.90_{-0.39}^{+0.36}$ & $0.67_{-0.34}^{+0.29}$ & < 1.52&$-2.96\pm0.46$ \\
180324 & $429.73_{-0.34}^{+0.34}$ & $0.79_{-0.35}^{+0.37}$ & $7.85_{-1.60}^{+1.67}$&$4.44\pm0.46$ \\
180417 & $474.65_{-0.15}^{+0.13}$ & $1.04_{-0.07}^{+0.07}$ & < 1.40&$-3.14\pm0.47$ \\
180430 & $264.10_{-0.03}^{+0.03}$ & $0.68_{-0.20}^{+0.12}$ & < 0.77&$-4.43\pm0.50$ \\
180515 & $354.86_{-0.21}^{+0.17}$ & $0.74_{-0.28}^{+0.24}$ & < 1.79&$-2.19\pm0.47$ \\
180525 & $387.57_{-0.15}^{+0.16}$ & $1.78_{-0.12}^{+0.13}$ & $3.75_{-0.58}^{+0.53}$&$5.22\pm0.48$ \\
180924 & $362.39_{-0.16}^{+0.16}$ & $0.75_{-0.10}^{+0.11}$ & < 2.28&$-1.61\pm0.47$ \\
181112 & $588.77_{-0.20}^{+0.19}$ & $0.57_{-0.14}^{+0.13}$ & < 1.71&$-4.36\pm0.47$ \\
190102 & $364.35_{-0.23}^{+0.21}$ & $0.45_{-0.20}^{+0.21}$ & < 1.69&$-2.44\pm0.46$ \\
190608 & $340.80_{-0.68}^{+0.64}$ & $2.30_{-0.59}^{+0.62}$ & $6.76_{-2.40}^{+2.07}$&$0.45\pm0.46$ \\
190611.2 & $321.29_{-0.89}^{+0.96}$ & $1.58_{-0.30}^{+0.30}$ & < 3.42&$-2.74\pm0.46$ \\
190711 & $590.46_{-0.73}^{+0.70}$ & $3.51_{-0.23}^{+0.24}$ & < 2.85&$-2.20\pm0.47$ \\
190714 & $503.86_{-0.31}^{+0.31}$ & $0.95_{-0.23}^{+0.19}$ & < 2.78&$-2.36\pm0.44$ \\

==> craft-scatter 200707/scatfit.tex <==
170107 & $608.38_{-0.82}^{+0.93}$& 571
 & $\mathit{0.98_{-0.35}^{+0.30}}$
 & ${0.79_{-0.45}^{+0.37}}$
 & ${< 1.31}$&$-8.8$ \\
170416 & $523.65_{-0.47}^{+0.50}$& 484
 & $\mathit{2.45_{-0.31}^{+0.37}}$
 & ${2.20_{-0.42}^{+0.39}}$
 & ${< 1.41}$&$-7.4$ \\
170428 & $992.45_{-0.78}^{+0.76}$& 952
 & $\mathit{<1.35}$
 & ${<1.38}$
 & ${< 1.44}$&$-10.5$ \\
170707 & $233.88_{-0.92}^{+0.87}$& 198
 & $\mathit{2.09_{-0.32}^{+0.37}}$
 & ${<0.89}$
 & ${< 0.71}$&$-33.6$ \\
170712 & $312.28_{-0.24}^{+0.30}$& 274
 & $\mathit{<0.80}$
 & ${<0.78}$
 & ${< 0.60}$&$-15.0$ \\
170906 & $389.15_{-0.88}^{+0.89}$& 350
 & $\mathit{0.99_{-0.34}^{+0.31}}$
 & ${0.82_{-0.29}^{+0.20}}$
 & ${< 0.54}$&$-8.7$ \\
171003 & $465.06_{-0.25}^{+0.23}$& 425
 & $\mathit{0.72_{-0.22}^{+0.19}}$
 & ${0.73_{-0.25}^{+0.19}}$
 & ${< 0.74}$&$-11.1$ \\
171004 & $303.78_{-0.35}^{+0.33}$& 265
 & $\mathit{0.85_{-0.29}^{+0.27}}$
 & ${0.65_{-0.36}^{+0.37}}$
 & ${< 1.12}$&$-18.4$ \\
171019{$^\dagger$} & $462.10_{-0.65}^{+0.74}$& 425
 & $\mathit{2.84_{-0.14}^{+0.15}}$
 & ${2.36_{-0.35}^{+0.37}}$
 & ${< 1.26}$&$-9.4$ \\
171020 & $114.01_{-0.11}^{+0.09}$& 76
 & $\mathit{<0.58}$
 & ${<0.53}$
 & ${< 0.39}$&$-8.3$ \\
171116 & $618.17_{-0.44}^{+0.46}$& 582
 & $\mathit{1.43_{-0.30}^{+0.31}}$
 & ${1.10_{-0.53}^{+0.43}}$
 & ${< 1.85}$&$-9.1$ \\
171213 & $158.42_{-0.07}^{+0.06}$& 122
 & $\mathit{<0.43}$
 & ${<0.47}$
 & ${< 0.35}$&$-6.3$ \\
171216 & $203.74_{-0.28}^{+0.32}$& 167
 & $\mathit{0.85_{-0.53}^{+0.37}}$
 & ${0.70_{-0.43}^{+0.45}}$
 & ${< 0.76}$&$-13.2$ \\
180110 & $714.03_{-0.27}^{+0.25}$& 675
 & ${4.73_{-0.21}^{+0.16}}$
 & $\mathit{<0.74}$
 & $\mathit{5.92_{-0.26}^{+0.27}}$ &$137.0$\\
180119 & $401.40_{-0.27}^{+0.26}$& 366
 & ${1.97_{-1.12}^{+0.60}}$
 & $\mathit{<0.56}$
 & $\mathit{1.94_{-0.33}^{+0.37}}$ &$1.4$\\
180128.0 & $441.34_{-0.44}^{+0.44}$& 409
 & $\mathit{1.27_{-0.26}^{+0.27}}$
 & ${0.72_{-0.41}^{+0.43}}$
 & ${< 1.72}$&$-5.0$ \\
180128.2 & $495.40_{-0.62}^{+0.61}$& 455
 & $\mathit{1.29_{-0.18}^{+0.19}}$
 & ${<0.77}$
 & ${< 2.95}$&$-1.8$ \\
180130 & $343.09_{-0.77}^{+0.76}$& 304
 & ${3.54_{-0.68}^{+0.82}}$
 & $\mathit{0.73_{-0.44}^{+0.56}}$
 & $\mathit{5.95_{-1.08}^{+1.33}}$ &$8.4$\\
180131 & $657.45_{-0.58}^{+0.53}$& 618
 & $\mathit{2.34_{-0.30}^{+0.32}}$
 & ${1.54_{-0.66}^{+0.67}}$
 & ${< 2.34}$&$-4.7$ \\
180212 & $167.56_{-0.11}^{+0.11}$& 137
 & $\mathit{<0.50}$
 & ${<0.45}$
 & ${< 0.28}$&$-10.0$ \\
180315 & $478.90_{-0.35}^{+0.35}$& 378
 & $\mathit{<0.89}$
 & ${<0.89}$
 & ${< 0.52}$&$-14.6$ \\
180324 & $429.73_{-0.35}^{+0.38}$& 366
 & ${2.72_{-0.46}^{+0.52}}$
 & $\mathit{<1.15}$
 & $\mathit{2.98_{-0.60}^{+0.62}}$ &$0.0$\\
180417 & $474.65_{-0.14}^{+0.15}$& 449
 & $\mathit{0.86_{-0.10}^{+0.10}}$
 & ${0.86_{-0.12}^{+0.11}}$
 & ${< 0.48}$&$-10.8$ \\
180430 & $264.11_{-0.04}^{+0.03}$& 95
 & $\mathit{<0.54}$
 & ${<0.58}$
 & ${< 0.24}$&$-12.2$ \\
180515 & $354.88_{-0.19}^{+0.18}$& 322
 & $\mathit{<0.76}$
 & ${<0.75}$
 & ${< 0.52}$&$-14.6$ \\
180525 & $387.49_{-0.14}^{+0.16}$& 357
 & ${2.24_{-0.09}^{+0.08}}$
 & $\mathit{1.65_{-0.15}^{+0.15}}$
 & $\mathit{1.30_{-0.21}^{+0.20}}$ &$0.8$\\
180924 & $362.38_{-0.15}^{+0.16}$& 322
 & $\mathit{0.66_{-0.13}^{+0.12}}$
 & ${<0.63}$
 & ${< 0.72}$&$-12.5$ \\
181112 & $588.76_{-0.20}^{+0.19}$& 549
 & $\mathit{<0.60}$
 & ${<0.58}$
 & ${< 0.55}$&$-8.7$ \\
190102 & $364.38_{-0.22}^{+0.20}$& 307
 & $\mathit{<0.67}$
 & ${<0.62}$
 & ${< 0.55}$&$-11.2$ \\
190608 & $339.48_{-0.51}^{+0.52}$& 302
 & $\mathit{3.45_{-0.29}^{+0.31}}$
 & ${2.22_{-0.64}^{+0.63}}$
 & ${< 3.58}$&$-6.2$ \\
190611.2 & $321.37_{-1.07}^{+0.96}$& 264
 & $\mathit{1.42_{-0.52}^{+0.45}}$
 & ${1.03_{-0.63}^{+0.61}}$
 & ${< 1.45}$&$-12.4$ \\
190711{$^\dagger$} & $590.49_{-0.79}^{+0.73}$& 534
 & $\mathit{3.47_{-0.24}^{+0.26}}$
 & ${3.32_{-0.35}^{+0.30}}$
 & ${< 1.12}$&$-8.2$ \\
190714 & $503.80_{-0.30}^{+0.30}$& 465
 & $\mathit{<0.88}$
 & ${<0.88}$
 & ${< 0.78}$&$-12.1$ \\

==> craft-scatter 200707/section4.tex <==


%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
	\includegraphics[trim={0 0 0 0 },clip,width=\columnwidth]{width_dm.pdf}%{CRAFT_RRATs_prediction.pdf}
    %\vspace{-8mm}
    \\
    \includegraphics[trim={0cm 0cm 0 0cm },clip,width=1.0\columnwidth]{scat_totaldm.pdf}%{CRAFT_RRATs_prediction.pdf}
    \\
	\includegraphics[trim={0cm 0cm 0 0cm },clip,width=1.0\columnwidth]{scat_ism.pdf}%{CRAFT_RRATs_prediction.pdf}
    \caption{Distribution of FRB pulse measurements against DM, confirmed measurements are plotted in blue, upperlimits are plotted in orange.
    \textit{Top:}
    Intrinsic width measurement ($\sigma$) and DM of ASKAP FRBs.
    \textit{Middle:}Scattering time ($\tau$) of ASKAP FRBs plotted against total DM,
    showing no correlation between the total DM and pulse broadening.
    \textit{Bottom:}Scattering time ($\tau$) of ASKAP FRBs plotted over estimated line of sight Galactic DM contribution from the NE2001 electron density model ($\mathrm{DM_{NE2001}}$).}
    \label{fig:width_dm}
    \label{fig:scat_ism}
    \label{fig:scat_total}
\end{figure}


%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
	\includegraphics[trim={0 0 0 0 },clip,width=\columnwidth]{freealpha_post_pub_version}%{CRAFT_RRATs_prediction.pdf}
    %\vspace{-8mm}
    \caption{Posterior distribution of FRB 180110 using a scattering model with an unconstrained scattering index. 
    The parameters shown are the centre position of pulse (t0/ms), scattering timescale at 1.3 GHz ($\tau$/ms), DM$_{\mathrm{err}}$ (DM offset/\dmunit), pulse width ($\sigma$/ms),
    $\alpha$ (alpha) and uncertainty (error). Priors for each parameter is displayed as a green curve. The three shades of contour correspond to 1,2 and 3\ $\sigma$ confidence level.
    }
    
    \label{fig:post_180110}
\end{figure}

%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
	\includegraphics[trim={0.9cm 3cm 0 3cm },clip,width=1.1\columnwidth]{freealpha_pub_version_residuals.pdf}%{CRAFT_RRATs_prediction.pdf}
    %\vspace{-8mm}
    \caption{Subband pulse profiles of FRB 180110. We plot the best-fitting model and residual for each subband. The exponential broadening scales with frequency using an exponential power law with an index of $-3.8$.}
    \label{fig:residual_180110}
\end{figure}

%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
	\includegraphics[trim={0 0 0 0 },clip,width=\columnwidth]{scat_dm_h.pdf}\\%{CRAFT_RRATs_prediction.pdf}
	%\includegraphics[trim={0 0 0 0 },clip,width=\columnwidth]{scat_dm_h2.pdf}\\%{CRAFT_RRATs_prediction.pdf}
	%\includegraphics[trim={0 0 0 0 },clip,width=\columnwidth]{scat_dm_h3.pdf}\\%{CRAFT_RRATs_prediction.pdf}
    %\vspace{-8mm}
    \caption{Pulse broadening measurement of ASKAP FRBs plotted against estimated extragalactic DM contribution. The scattering time, $\tau$ is scaled to 1.3 GHz with a power law index of --$4$. The population inference fit results from the flat model is plotted as an estimate limit of the scattering, the $1-\sigma$ upper limit and $2-\sigma$ lower limits is displayed as the shaded region in red. The scaled DM$-\tau$ relation from \citet{2019ARA&A..57..417C} is drawn with $1-\sigma$ uncertainty shaded region in green. We display the DM$-\tau$ relation of Galactic pulsars from \citet{2004ApJ...605..759B} and the measure of scattering from Galactic pulsars \citep{2005AJ....129.1993M} as comparison of the scattering expected from Milky-Way-like ISM.}
    \label{fig:scat_dm}
\end{figure}

%%%%%%%%%%%%%%%%







